A Complete List of All Convex Polyhedra Made by Gluing Regular Pentagons

We give a complete description of all convex polyhedra whose surface can be constructed from several congruent regular pentagons by folding and gluing them edge to edge. Our method of determining the graph structure of the polyhedra from a gluing is of independent interest and can be used in other similar settings.

==> figs/6all.tex <==
\centering
\def\fltnn#1#2#3{( #1 cm - 0.38 * #2 cm, #3 cm - 0.2 * #2 cm)}

\tikz[scale=1.85]{
\def\a{\fltnn{1.4310957967719642}{0.0}{0.0} node{ }}
\def\b{\fltnn{0.7162308035620336}{0.3787815383028905}{-0.587786175174265} node{ }}
\def\c{\fltnn{-0.7155478984982786}{0.0}{-1.2393653153906468} node{ }}
\def\d{\fltnn{-0.8671531615396659}{0.3787815383070919}{-0.3263809830922096} node{ }}
\def\e{\fltnn{-0.7155478985611488}{-0.0000000003687175}{1.2393653153533593} node{ }}
\def\f{\fltnn{0.15092235791116757}{0.3787815381579165}{0.9141671585035448} node{ }}
\def\g{\fltnn{0.0}{0.7549741064176964}{0.0} node{ }}
\def\h{\fltnn{0.15092235791177575}{-0.3787815383030031}{-0.9141671584442804} node{ }}
\def\i{\fltnn{-0.8671531614092768}{-0.37878153847290486}{0.3263809832477606} node{ }}
\def\j{\fltnn{0.7162308035616037}{-0.37878153839618434}{0.5877861751136217} node{ }}
\def\k{\fltnn{0.0}{-0.7549741069521263}{0.0} node{ }}

\draw [color=thr, dashed] \e -- \g -- \a -- \f;
\draw [color=thr, dashed] \g -- \c -- \b;

\draw [thick,color=edThr, dashed] \j -- \f -- \g -- \b;
\draw [thick,color=edThr, dashed] \e -- \f;
\draw [thick,color=edThr, dashed] \g -- \d;

\zal 1 \c -- \d -- \i -- \k -- \h -- cycle;
\zal 2 \b -- \h -- \k -- \j -- \a -- cycle;
\zal 4 \j -- \k -- \i -- \e -- cycle;
\zal 3 \e -- \i -- \d -- cycle;

\draw \h -- \b -- \a -- cycle;
\draw \i -- \d -- \c -- cycle;
\draw \i -- \e -- \d -- cycle;
\draw \k -- \h -- \a -- cycle;
\draw \k -- \c -- \h -- cycle;
\draw \k -- \i -- \c -- cycle;
\draw \k -- \e -- \i -- cycle;
\draw \k -- \j -- \e -- cycle;
\draw \k -- \a -- \j -- cycle;

\draw [thick,color=edHr] \e -- \i -- \k -- \j;
\draw [thick,color=edHr] \a -- \j -- \k -- \h -- \b -- cycle;
\draw [thick,color=edHr] \h -- \c -- \d -- \i -- \k -- cycle;

%
	\draw \k node[above]{$U$};
	\draw \g node[below]{$V$};
%
	\draw \j node[above]{$C_1$};
	\draw \i node[left]{$C_2$};
	\draw \h node[below]{$C_3$};
%
	\draw \d node[left]{$D_1$};
	\draw \b node[right]{$D_2$};
	\draw \f node{$D_3$};
%
	\draw \c node[below]{$F_2$};
	\draw \a node[right]{$F_3$};
	\draw \e node[left]{$F_1$};
}
	\caption{Shape 6.}
	\label{fig:6all}

==> figs/diagdiv.tex <==
\centering
\tikz[scale=1.25]{
	\filldraw [thick, fill opacity=0.55, fill=fill4] (90:1.4) -- (162:1.4)
		-- (234:1.4) -- (306:1.4) -- (18:1.4) -- cycle;
	\draw [thick,dashed] (306:1.4) -- (162:1.4);
	\draw [thick] (234:1.4) -- (18:1.4);
	
	\draw (306:1.65) node{$U$};
	\draw (18:1.65) node{$C_1$};
	\draw (234:1.65) node{$C_2$};
	\draw (162:1.65) node{$F_1$};
	\draw (90:1.65) node {$D_3$};
	\draw (0,-0.26) node{$X$};

	\draw (-0.42,-1.5) node[below]{$\xi = 1 / (2 \cdot \cos(36^\circ))^2$};
	\draw [->] (-0.42,-1.6) -- (-0.42,-0.9);

	\draw (1.5,-0.18) node[right]{$1 - 1 / (2 \cdot \cos(36^\circ))^2$};
	\draw [->] (1.55,-0.18) -- (0.62,-0.18);
}
\caption{The ratio the diagonals are divided with.}
\label{fig:diagdiv}

==> figs/shortCorr.tex <==
\begin{figure}[h] \centering \tikz[scale=1.24]{
	\coordinate (dp) at (0.12 * 1.5, 0.12 * 2);
	\filldraw[thick,fill=fill2,fill opacity=0.55,xshift=0.12 cm,yshift=0.2 cm]
	     (-0.5,-1.25) to[out=0,in=255] (1.6,0.25) to[out=75,in=-20] (1.4,1.6)
	     to[out=165,in=65] (-1.4,-0.08) to[out=245,in=180] (-0.5,-1.25);
	\draw[thick,color=highlight] (0,0) -- (1.05,1.4);
	\fill[fill=black] (0,0) circle[radius=0.44mm] node[below]{$v_i$}
	     (1.05,1.4) circle[radius=0.44mm] node[above]{$v_j$};
	\draw (1.5,-0.95) node{$M$};
\begin{scope}[xshift=-4.8cm,yshift=0.35cm]
	\coordinate (dp) at (0.12 * 1.5, 0.12 * 2);
	\filldraw[thick,fill=fill4,fill opacity=0.55] (1.05,1.4) -- (0.3,1.15) -- (-1.5,-0.5) --
	     (-0.5,-1.25) -- (1,-1) -- (1.8,0.9) -- cycle;
	\draw[thick] (-1.5,-0.5) -- (0,0) -- (1,-1);
	\draw[thick,color=red] (0,0) -- (dp);
	\draw[thick,color=highlight] (dp) -- (1.05,1.4);
	\draw (dp) ++(-0.03*2,0.03*1.5) -- ++(0.06*2,-0.06*1.5);
	\draw (0.066 * 1.5, 0.04 * 2) node[right]{$\le \mu$};
	\draw (0,0) node[below]{$u_i$} (1.05,1.4) node[above]{$u_j$} (-1.5,-1.25) node{$P$};
\end{scope} }
	\caption{Edges in $P$ correspond to shortest paths in $M$, their lengths differ by at most $\mu$.}
	\label{fig:shortCorr}
\end{figure}


==> figs/thrvert.tex <==
\centering
\tikz[scale=0.87]{
\begin{scope}[yscale=0.4,xscale=1]
	\draw[dotted] (0,0) circle[radius=2.5cm];

	\coordinate (Q) at (20:2.5cm);
	\coordinate (W) at (140:2.5cm);
	\coordinate (E) at (260:2.5cm);
	\coordinate (R) at (0,4.5);

	\draw[thick,dashed] (Q) -- (W);
	
	\filldraw[draw=black,fill=fill1,fill opacity=0.55] (R) -- (E) -- (W) -- cycle;
	\filldraw[draw=black,fill=fill2,fill opacity=0.55] (R) -- (E) -- (Q) -- cycle;
	
	\draw[thick] (Q) -- (R) -- (W) -- (E) -- cycle;
	\draw[thick] (R) -- (E);

	\draw (Q) node[right]{$C_1 = (\sin\alpha, 0, -\cos\alpha)$};
	\filldraw (Q) circle[radius=0.08cm];

	\draw (W) node[left]{$C_2 = (
		-\frac{\sin\alpha}{2},
		\frac{\sqrt 3 \sin\alpha}{2},
		-\cos\alpha
	)$};
	\filldraw (W) circle[radius=0.08cm];

	\draw (E) node[below]{$C_3 = (
		-\frac{\sin\alpha}{2},
		-\frac{\sqrt 3 \sin\alpha}{2},
		-\cos\alpha
	)$};
	\filldraw (E) circle[radius=0.08cm];

	\draw (R) node[above]{$U=(0,0,0)$};
	\filldraw (R) circle[radius=0.08cm];
\end{scope}
}
    
\caption{Coordinates of vertices $U$, $C_1$, $C_2$, $C_3$.}
\label{fig:thrvert}

==> graphics/1.tex <==
\tikz{
	\filldraw[draw=edHr,thick,fill=fill1,fill opacity=0.55,rotate=34]
	(0:0.95cm) -- (72:0.95cm) -- (144:0.95cm) -- (216:0.95cm) -- (288:0.95cm) -- cycle;
}

==> graphics/cube.tex <==
\begin{center} \tikz{
\def\a{\fltn{0}{0}{0}}
\def\e{\fltn{0}{0}{1}}
\def\d{\fltn{0}{1}{0}}
\def\h{\fltn{0}{1}{1}}
\def\b{\fltn{1}{0}{0}}
\def\f{\fltn{1}{0}{1}}
\def\c{\fltn{1}{1}{0}}
\def\g{\fltn{1}{1}{1}}

\draw \a -- \b -- \c -- \d -- cycle;
\draw \h -- \e -- \f -- \g -- cycle;
\draw \a -- \e; \draw \b -- \f; \draw \c -- \g; \draw \d -- \h;
} \end{center}
